Exploring new features of neutrino oscillations with very low energy monoenergetic neutrinos

In the present work we propose to study neutrino oscillations employing sources of monoenergetic neutrinos following electron capture by the nucleus. Since the neutrino energy is very low the smaller of the two oscillation lengths, L23, appearing in this electronic neutrino disappearance experiment can be so small that the full oscillation can take place inside the detector and one may determine very accurately the neutrino oscillation parameters. Since in this case the oscillation probability is proportional to theta13, one can measure or set a better limit on the unknown parameter theta13. This is quite important, since, if this mixing angle vanishes, there is not going to be CP violation in the leptonic sector. The best way to detect it is by measuring electron recoils in neutrino-electron scattering. One, however, has to pay the price that the expected counting rates are very small. Thus one needs a very intensive neutrino source and a large detector with as low as possible energy threshold and high energy and position resolution. Both spherical gaseous and cylindrical liquid detectors are studied. Different source candidates are considered.

==> begin.tex <==
\newcommand{\p}{\partial}
\newcommand{\ls}{\left(}
\newcommand{\rs}{\right)}
%\newcommand{\beq}{\begin{equation}}
%\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\bdm}{\begin{displaymath}}
\newcommand{\edm}{\end{displaymath}}
\newcommand{\fps}{f_{\pi}^2 }
\newcommand{\mks}{m_{{\mathrm K}}^2 }
\newcommand{\ms}{m_{{\mathrm K}}^{*} }
\newcommand{\msq}{m_{{\mathrm K}}^{*2} }
\newcommand{\rhos}{\rho_{\mathrm s} }
\newcommand{\rhob}{\rho_{\mathrm B} }
\newcommand{\Jb}[2]{J_{#1} (k#2)}
\newcommand{\kro}[1]{\delta_{#1}}
\newcommand{\equa}[1]{(\ref{#1})}
\newcommand{\equas}[2]{(\ref{#1}--\ref{#2})}
\newcommand{\order}[1]{{\cal O} \left( #1 \right )}
\newcommand{\cO}[1]{{\cal O} \left( #1 \right )}
\newcommand{\lesim}{\mbox{\raisebox{-.6ex}{$\,{\stackrel{<}{\sim}}\,$}}}
\newcommand{\gesim}{\mbox{\raisebox{-.6ex}{$\,{\stackrel{>}{\sim}}\,$}}}
\newcommand{\semiclass}{\ \stackrel{\rm s.c.}{\longrightarrow}\ }
\renewcommand{\thefootnote}{\#\arabic{footnote}}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\renewcommand{\thetable}{\thesection.\arabic{table}}
\renewcommand{\arraystretch}{1.2}








